On Ranking Consistency of Pre-ranking Stage

Industrial ranking systems, such as advertising systems, rank items by aggregating multiple objectives into one final objective to satisfy user demand and commercial intent. Cascade architecture, composed of retrieval, pre-ranking, and ranking stages, is usually adopted to reduce the computational cost. Each stage may employ various models for different objectives and calculate the final objective by aggregating these models' outputs. The multi-stage ranking strategy causes a new problem - the ranked lists of the ranking stage and previous stages may be inconsistent. For example, items that should be ranked at the top of the ranking stage may be ranked at the bottom of previous stages. In this paper, we focus on the \textbf{ranking consistency} between the pre-ranking and ranking stages. Specifically, we formally define the problem of ranking consistency and propose the Ranking Consistency Score (RCS) metric for evaluation. We demonstrate that ranking consistency has a direct impact on online performance. Compared with the traditional evaluation manner that mainly focuses on the individual ranking quality of every objective, RCS considers the ranking consistency of the fused final objective, which is more proper for evaluation. Finally, to improve the ranking consistency, we propose several methods from the perspective of sample selection and learning algorithms. Experimental results on one of the biggest industrial E-commerce platforms in China validate the efficacy of the proposed metrics and methods.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> deploy.tex <==
\section{Online Serving}
\subsection{Challenges}
\subsection{Solution}
\begin{itemize}
	\item sequence cutoff and feature dim reduction
	\item less orders
	\item kernel optimazation
\end{itemize}
\subsection{Results}

==> experiments.tex <==
\begin{table*}[t]
	\caption{The example percentage of each domain.}
	\label{table:sample_percentage}
	\resizebox{\textwidth}{!}{\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
	\toprule
	         &1 & 2& 3& 4& 5& 6& 7& 8& 9& 10& 11& 12& 13& 14& 15& 16& 17& 18& 19\\
	\midrule
	Percentage &0.99\% & 1.61\% &3.40\% &3.85\% &2.79\% &0.56\% &4.27\% &16.76\% &10.00\% &12.16\% &0.76\% &1.31\% &3.34\% &28.76\% &1.17\% &0.46\% &1.05\% &0.91\% &5.85\%   \\
	\bottomrule
	\end{tabular}}
\end{table*}
\section{Experiments}

We evaluate the efficacy of STAR in this section. We begin by introducing the setup including the used production dataset, compared method and implementation details in Sec.~\ref{sec:setting}.  The results and discussion are elaborated in Sec.~\ref{sec:res}. We also perform in-depth ablation studies in Sec.~\ref{sec:ablation}. Experimental results on production environment are shown in Sec.~\ref{sec:industrial}.

\subsection{Experimental Settings}\label{sec:setting}



\textbf{Dataset.} We use Alibaba production data regarding user click behavior on 19 business domains to perform the offline evaluation.  The training data is collected from traffic logs of the online display advertising system of Alibaba. Data of one day from 19 business domains are used for training and the data of the following day is used for testing. The training dataset consists of  billions of examples. \ref{table:sample_percentage} shows the example percentage of each domain in the training set.


\textbf{Compared models.}
To verify the effectiveness of the proposed approach, we compare STAR with the following models:
\begin{itemize}
    \item \textbf{Base}. We refer to Base as the model composed of embedding layer, pooling \& concatenation layer, batch normalization and a 7-layer fully-connected networks. Specifically, the pooling \& concatenation layer is based on DIEN~\cite{zhou2019dien}, which extracts user interest after the embedding layer. After the extraction. We mix all samples from different domains and train the base model.
    \item \textbf{Shared Bottom}. The Shared Bottom model is a multi-task model that shares the parameters of bottom layers. In our implementation, we let the Shared Bottom share the embedding layer and interest extraction layer. Each domain will also have a specific 7-layer fully-connected network that is not shared.
    \item \textbf{MMoE}. MMoE~\cite{MaZYCHC2018MMOE} implicitly models task relationship for multi-task learning, where different tasks may have different label spaces. Here we adapt MMoE for multi-domain CTR prediction, where each  fully-connected network is treated as an expert. The number of expert is equal to the number of domains. Besides, MMoE also learns   gating networks per domain that takes the input features and outputs softmax gates assembling the experts with different weights. 
\end{itemize}
To give a fair comparison, all compared methods and the STAR model are trained with the proposed auxiliary network in Sec.~\ref{sec:res}. The ablation study about the auxiliary network is performed in Sec.~\ref{sec:ablation}.

\textbf{Implementation details.} 
All models are trained with Adam~\cite{KingmaB2014Adam}, the learning rate is set to 0.001 and the batch size is 2000. We minimize the cross-entropy loss for samples from all domains to train the model.

\textbf{Metrics.} 
Area under the ROC curve (AUC) is the common metric used to evaluate the performance of CTR prediction. An variation of user weighted AUC~\cite{zhou2018din}  measures the goodness of intra-user order by averaging AUC over users and is shown to be more relevant to online performance in display advertising system. It is calculated as follows:
\begin{equation}
    \textrm{AUC} = \frac{\sum_i^n \# \textrm{impression}_i \times \textrm{AUC}_i}{\sum_i^n \# \textrm{impression}_i},
\end{equation}
where $n$ is the number of users, $\textrm{impression}_i$ and $\textrm{AUC}_i$ are the number of impressions and AUC of the $i$-th user, respectively. 
We use this weighted AUC as the evaluation metric and still refer it as AUC for simplicity. Concretely, we use the AUC of each domain and overall AUC (mixing samples from all domains to calculate the overall AUC) as the metrics.  

\subsection{Results}\label{sec:res}
We evaluate all approaches on Alibaba production dataset. To give a fair comparison, all compared methods and the STAR model are trained with the proposed auxiliary network. The result is shown in  Table~\ref{table:offline_result}. As illustrated in Table~\ref{table:offline_result}, 
the Shared Bottom model, MMoE and STAR all achieve better overall performance than Base model. This demonstrate the importance of exploiting domain relationship and capturing domain distinction to enhance the prediction performance. The consistent improvement validates the efficacy of STAR. 

Although the Shared Bottom and MMoE achieve better overall performance than the Base model, note that in some domains, the performance of Shared Bottom and MMoE is worse than the Base model, e.g., domain \# 5 and \#16.
In contrast, the proposed STAR model exhibits superior performance across all domains comparing with the Base model. Besides, STAR also achieves consistent improvement than the Shared Bottom, which demonstrates the importance of information sharing on top layers for multi-domain learning where all domains shares the same label space. STAR also outperforms MMoE, which shows the superiority of explicitly model domain relationship compared with implicitly implicitly model domain relationship by the gate networks. 


% \begin{table}[t]
% 	\caption{Results of different approaches on offline production dataset.}
% 	\label{table:offline_result}
% 	\begin{tabular}{c|c|c|c|c}
% 	\toprule
% 	        & Base & Multi-Head & MMoE & STAR \\
% 	\midrule
% 	\#1           &0.6134&0.6103 &0.6135                     & 0.6306       \\
% 	\#2           &0.6321&0.6258 &0.6323 & 0.6417        \\
% 	\#3           &0.6281&0.6238 &0.6282 & 0.6372        \\
% 	\#4           &0.6326&0.6301 &0.6328 & 0.6451        \\
% 	\#5           &0.6308&0.6230 &0.6302 & 0.6388        \\
% 	\#6           &0.6378&0.6342 &0.6359 & 0.6494        \\
% 	\#7           &0.6305&0.6278 &0.6305 & 0.6410        \\
% 	\#8           &0.6297&0.6278 &0.6295 & 0.6411        \\
% 	\#9           &0.6264&0.6237 &0.6262 & 0.6368        \\
% 	\#10           &0.6392&0.6348 &0.6359 & 0.6577 \\
% 	\#11          &0.6469 &0.6404 &0.6434 & 0.6719        \\
% 	\#12           &0.6506&0.6464 &0.6461& 0.6676        \\
% 	\#13           &0.6558&0.6527 &0.6530& 0.6739        \\
% 	\#14           &0.6362&0.6360 &0.6370& 0.6486        \\
% 	\#15           &0.6043&0.5577 &0.5918& 0.5851        \\
% 	\#16           &0.6745&0.6769 &0.6696 & 0.7021        \\
% 	\#17           &0.6638&0.6684 &0.6491& 0.6901        \\
% 	\#18           &0.6524&0.6581 &0.6476 & 0.6715        \\
% 	\#19           &0.6493&0.6480 &0.6352 & 0.6754        \\
% 	\#20           &0.6330&0.6304 &0.6297 & 0.6476        \\
% 	\midrule
% 	Average AUC            & 0.000 &0 & &  0.000       \\
% 	Overall AUC & 0.6364 &0.6343 & 0.6345& 0.6506        \\
% 	\bottomrule
% 	\end{tabular}
% \end{table}

\begin{table}[t]
	\caption{Results of different approaches on offline Alibaba production dataset.}
	\label{table:offline_result}
	\begin{tabular}{c|c|c|c|c}
	\toprule
	        & Base & Shared Bottom & MMoE  & STAR \\
	\midrule
	\#1
	&0.6134&0.6186&0.6143& \textbf{0.6306 }      \\
	\#2
	&0.6321&0.6320&0.6355 & \textbf{0.6417}        \\
	\#3           &0.6281&0.6293&0.6311 & \textbf{0.6372}        \\
	\#4 &0.6326&0.6361&0.6373 & \textbf{0.6451}        \\
	\#5
	&0.6308&0.6292&0.6336& \textbf{0.6388}        \\
	\#6
	&0.6378&0.6383 &0.6412& \textbf{0.6494}        \\
	\#7
	&0.6305&0.6329 &0.6340& \textbf{0.6410}        \\
	\#8
	&0.6297&0.6278 &0.6330&\textbf{0.6411}        \\
	\#9
	&0.6264&0.6283&0.6292& \textbf{0.6368}        \\
	\#10
	&0.6392&0.6434 &0.6431& \textbf{0.6577} \\
	\#11
	&0.6469 &0.6529&0.6508& \textbf{0.6719}        \\
	\#12
	&0.6506&0.6575
	& 0.6518&\textbf{0.6676}        \\
	\#13
	&0.6558&0.6612 &0.6603& \textbf{0.6739}        \\
	\#14
	&0.6362&0.6405 &0.6412& \textbf{0.6486}        \\
% 	\#15
% 	&0.6043&0.5739 &0.6207& 0.5851        \\
	\#15
	&0.6745&0.6888 &0.6787& \textbf{0.7021}        \\
	\#16&0.6638&0.6627 &0.6634& \textbf{0.6901}        \\
	\#17&0.6524&0.6658 &0.6519& \textbf{0.6715}        \\
	\#18 &0.6493&0.6480&0.6500 & \textbf{0.6754}        \\
	\#19 &0.6330&0.6375&0.6374 & \textbf{0.6476}        \\
	\midrule
% 	Average AUC & 0.000 &0  &  0.000 &0.000      \\
	Overall AUC & 0.6364 & 0.6398 &0.6403 & \textbf{0.6506}        \\
	\bottomrule
	\end{tabular}
\end{table}

\subsection{Ablation Study}\label{sec:ablation}

To investigate the effect of each component, we conduct several ablation studies.



































































































\subsubsection{STAR FCN and PN} 

\begin{table}[t]
	\caption{Ablation study of partitioned normalization (PN) and star topology fully-connected neural networks (STAR FCN). All models are trained with the proposed auxiliary network.}
	\label{table:ablation_shadow}
	\resizebox{\columnwidth}{!}{\begin{tabular}{c|c|c|c|c}
	\toprule
	  &    Base (BN)  & Base (PN) & STAR FCN (BN) & STAR FCN (PN) \\
	\midrule
% 	Average AUC           & 0.000 &0.000&0.000&0.000\\
	Overall AUC & 0.6364 &0.6485 & 0.6415 &  \textbf{0.6506}    \\
	\bottomrule
	\end{tabular}}
\end{table}
We analyze the influence of different components of STAR. Concretely, the separate effects of star topology fully-connected neural networks (STAR FCN)  and partitioned normalization (PN) are investigated. We compare the Base model trained with BN, Base model trained with PN, STAR FCN with BN and the STAR model (STAR FCN + PN). The result is reported  in Table~\ref{table:ablation_shadow}. 
We observe that using only shadow brings xx\% improvement and using only SSLT brings xx\% improvement. Bring them together improves XX\% compared with the Base model. The result validates the effect of both STAR FCN and PN.

\subsubsection{Normalization}
Normalization methods are very effective component in deep learning, which have been shown by many practices to ease optimization and enable very deep networks to converge. We analyze the effect of different normalization methods including Batch Normalization (BN)~\cite{PiBZZG19MIMN}, Layer Normalization (LN)~\cite{BaKH2016LN} and the proposed Partitioned Normalization (PN) on multi-domain CTR prediction. BN accumulates global statistics and learns global parameters for samples from all domains. LN is a representative instance-based normalization method, which operates along the channel dimension and avoid mixing statistics for samples from different domains. 

The result is shown in Table~\ref{table:ablation_normalization}.
Our first observation is that both LN and PN outperforms BN. This observation validates that data from different domains have distinct distribution. Thus  global normalization methods obscure domain differences. which will not perform well on multi-domain CTR prediction.
We find PN outperforms LN, this validates that  privatizing normalization for samples from different domains outperforms operating normalization  only for each sample since PN leads to more accurate moments.

\begin{table}[t]
	\caption{Ablation study of normalization methods for multi-domain CTR prediction. STAR FCN is trained BN, LN and PN respectively.}
	\label{table:ablation_shadow}
	\resizebox{\columnwidth}{!}{\begin{tabular}{c|c|c|c}
	\toprule
	  &STAR FCN (BN) &    STAR FCN (LN) & STAR FCN (PN) \\
	\midrule
% 	Average AUC           & 0.000 &0.000&0.000&0.000\\
	Overall AUC &0.6415 & 0.6463 &  \textbf{0.6506}    \\
	\bottomrule
	\end{tabular}}
\end{table}

\subsubsection{Auxiliary network} 
We conduct experiment to assess the effect of auxiliary network for different models. Base model, Shared Bottom model, MMoE and STAR are trained with and without auxiliary network. The result is illustrated in Figure~\ref{fig:ablation_auxiliary}. We observe that auxiliary network improves base model, Shared Bottom model,  MMoE and STAR consistently. The result  validates the importance of making full utilization of domain features and capturing the domain distinction.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figure/eval_aux.pdf}
    \caption{The performance of different methods trained without and with auxiliary network.}
    \label{fig:ablation_auxiliary}
\end{figure}

% \textbf{Normalization} 
% \begin{table}[t]
% 	\caption{The effect of different  normalization methods.}
% 	\label{table:ablation_normalization}
% 	\begin{tabular}{c|c|c|c|c}
% 	\toprule
% 	  &    BN   & LN & SBN  \\
% 	\midrule
% 	Average AUC           & 0.000 &0.000&0.000\\
% 	Overall AUC  &0.000&0.000 &0.000      \\
% 	\bottomrule
% 	\end{tabular}
% \end{table}


\subsection{Production}\label{sec:industrial}
\textbf{Online serving and challenges.} 
One of the challenges in industrial recommender is that the distribution of features and click through rate (CTR) exhibits large shifts over time. 
To capture the dynamic change of data in real time, it is important to use the real-time examples to update the CTR models continuously to prevent them from becoming stale. 
% The common way to organize input data for CTR prediction is to abstract data in the domain-level. The domain-level abstraction treats each domain independently and organizes domain-specific data for each domain. To combine data from multiple domains, it needs large development cost. If we want to add new domains and combine data from different sources, it need re-develop a new dataflow to construct the input data. The re-development is both inefficient and time-consuming, which is due to the lack of flexibility and information reuse.To address this issue, we optimize the online data flow where basic data unit flow as the minimal unit and takes it as input dataflow. Different input dataflows can be split and assembled flexibly for different tasks. This implementation enables efficient algorithm iteration on online data from multiple business domains.
However, for multi-domain CTR prediction, the real-time example percentage of each domain changes over time. For example, some business domains have  traffic spike on morning while  some business domains have  traffic spike on evening. If we mix real-time samples from all domains for each mini-batch according to chronological order, the changes of data percentage over time will cause the instability of model learning. To address this issue, we redesign the data pipeline, where each batch only contain examples from a single business domain. Besides, we maintain a buffer that store history samples. Samples are shuffled and then  feed to the model to avoid the sudden change of example percentage. After that, this mini-batch of samples are removed from the buffer. We empirically found this training manner is more stable than the traditional way of online update. 


The systematical optimization makes STAR capable of serving main traffic from multiple business domains stably. Table~\ref{tab:production} shows the improvement of STAR on the display advertising system of Alibaba. We compute the overall improvements on all domains. The introduction of STAR brings +8.0\% overall CTR lift and +6.0\% overall RPM (Revenue Per Mille) lift in our online A / B test compared with the Base model. 
\begin{table}[t]
	\caption{CTR and RPM gains in online display advertising system of Alibaba.}
	\label{tab:production}
	\begin{tabular}{l|l|l}
	\toprule
	         & CTR & RPM \\
	\midrule
	Overall   & +8.0\%  & +6.0\% \\
	\bottomrule
	\end{tabular}
\end{table}





==> related.tex <==
\section{Related Work}
In this section, we list and compare several works that are relevant to us.
% Finally are the discussion of the ranking consistency of different stages.

%\subsection{Multi-Stage Ranking System}

%\subsection{Retrieval}
%The goal of the retrieval stage is to generative a small subset of candidate items for the ranking stage. Embedding-based Retrieval (EBR) has been applied in industrial systems for years~\cite{CovingtonAS2016YouTubeDNN,HuangSSXZPPOY2020FacebookEBR,WangHZZZL2018TaobaoEmbedding,GrbovicC2018AirbnbEmbedding}.
%As an early representative work,  YouTube video recommender systems use a neural network to project users and items into low-dimensional embeddings and measure the user-item preference by the inner-product. At serving, an approximate nearest neighbor lookup is performed to generate candidate items. Facebook Search system introduce the unified embedding framework developed to model semantic embeddings for personalized search, and share experiences on optimization of the ranking system~\cite{HuangSSXZPPOY2020FacebookEBR}.

%Due to the limited learning capacity of EBR model, MIND~\cite{Li2019MIND} use capsule network and the dynamic routing mechanism to learn multiple representations. To break the bottleneck of inner-product preference modeling, tree-based retrieval methods~\cite{zhu2018tdm,ZhuCXZLHLXG2019JTM} are proposed to take a tree structure as index. TDM~\cite{zhu2018tdm} provide logarithmic complexity w.r.t. corpus size even with more expressive models such as deep neural networks.


%\subsection{Ranking}
%In industrial recommender, the ranking stage ranks the items considering multiple objectives. Learning to Rank (LTR) is a fundamental problem for recommender system~\cite{GuSTRL2015RankingSVM,BurgesSRLDHH2005RankNet,CaoQLTL2007ListNet}. In the pairwise approach, the learning task is formalized as
%classification of object pairs into correctly ranked and incorrectly ranked categories~\cite{GuSTRL2015RankingSVM,BurgesSRLDHH2005RankNet}. In the listwise approach, lists instead of document pairs are used as instances in learning~\cite{CaoQLTL2007ListNet}.

%Since industrial systems often need accurate click-through rate (CTR) and conversion rate (CVR) prediction. Pointwise approach are also widely used. In recent years, there is a growing number of research studying modeling CTR/CVR with deep neural networks~\cite{CovingtonAS2016YouTubeDNN,zhou2018din,PiZZWRFZG2020SIM,FengLSWSZY19DSIN,MaZHWHZG2018ESMM,GuSFZZ2021Defer,YangLHZZZT2020ESDFM}. The final rank scores is obtained by fusing multiple objectives such as CTR, CVR, watch-time.  
